CasCast: Skillful High-resolution Precipitation Nowcasting via Cascaded Modelling

Precipitation nowcasting based on radar data plays a crucial role in extreme weather prediction and has broad implications for disaster management. Despite progresses have been made based on deep learning, two key challenges of precipitation nowcasting are not well-solved: (i) the modeling of complex precipitation system evolutions with different scales, and (ii) accurate forecasts for extreme precipitation. In this work, we propose CasCast, a cascaded framework composed of a deterministic and a probabilistic part to decouple the predictions for mesoscale precipitation distributions and small-scale patterns. Then, we explore training the cascaded framework at the high resolution and conducting the probabilistic modeling in a low dimensional latent space with a frame-wise-guided diffusion transformer for enhancing the optimization of extreme events while reducing computational costs. Extensive experiments on three benchmark radar precipitation datasets show that CasCast achieves competitive performance. Especially, CasCast significantly surpasses the baseline (up to +91.8%) for regional extreme-precipitation nowcasting.

==> backup2.tex <==
\subsection{Conditional Diffusion in Latent Space}
We employ diffusion in the latent space for high-resolution precipitation nowcasting generation in the probabilistic component of CasCast. Diffusion models do not exhibit mode collapse and artifacts compared with forecasting methods using GANs. Additionally, latent space enables efficient training and sampling in the diffusion-based precipitation nowcasting.

\textbf{Preliminary of Diffusion Models.} Diffusion models learn the reverse process of gradually noising data $x_{0}$ into Gaussian noise. By progressively denoising the Gaussian noise, diffusion models generate samples $\hat{x} ~ \sim p(x_{0})$ where $p(x_{0})$ is data distribution. The noising process is a Markov process defined as $q(x_{k}|x_{k-1})=N(x_{k}; \sqrt{\alpha_{k}}x_{k-1}, \beta_{k}I), 1\leq k \leq K$ where $\beta_{k}=1-\alpha_{k}$ and $\alpha_{k}$ is  the $k^{th}$ step's constant coefficient of noise schedule. When $x_0 \sim p(x_{0})$ is given, the distribution of $x_{k}$ can be derived as $q(x_{k}|x_0)=N(x_{k}; \sqrt{\Bar{\alpha_k}}x_{0}, \sqrt{1-\Bar{\alpha_k}}I)$. In the denoising process, the joint distribution $p_{\theta}(x_{0:K})$ is factorized into multiplications of conditional distribution $p_{\theta}(x_{0:K}) = p(x_K) \prod_{i=K}^{i=1} p_{\theta}(x_{i-1}|x_{i})$. Diffusion models, parameterized as $\theta$, iteratively estimate $x_{k-1}$ from $p_{\theta}(x_{k-1}|x_{k})$ using MAE (maximum likelihood estimation). Finally, Gaussian noise $x_K$ is denoised into data sample $x_0$.

\textbf{Framewise Autoencoder.}
It is difficult to directly apply the high-dimensional radar data, on which precipitation nowcasting heavily depending, to the training and sampling of diffusion models. On the one hand, the radar echos, typically spanning several hours with a time interval of five minutes, composes a long sequence. On the other hand, most radar data with a high resolution (such as 1km) cover areas within a radius of hundreds of kilometers ~\cite{shi2017deep, veillette2020sevir, Gwennaelle2020meteonet}. Therefore, it is extremely challenging to directly generate short-term precipitation forecasts in pixel space with diffusion, due to the high dimension property of radar data. Another characteristic of radar data is redundancy. Radar echo usually contains redundant background intensity as the situation, where precipitation is continuous and consistent over a  coverage area of several hundred kilometers, is rare. The redundancy and high dimensionality exhibited in radar data motivate us to use a framewise autoencoder for the compression of radar data. We follow ~\cite{rombach2022high} to train a framewise autoencoder with pixel-wise loss and adversarial loss. Specifically, frame encoder $\mathrm{E}$ is trained to encode radar echo frame $x\in R^{1 \times C \times H \times W}$ into latent representation $\mathrm{E}(x) \in R^{1 \times C_z \times H_z \times W_z }$. The decoder reconstructs data frame $\hat{x}=\mathrm{D}(\mathrm{E}(x))$ from the latent representation. The latent space accelerates the training and sampling of diffusion models without severely corrupting the accuracy of prediction.

As shown in ~\cref{fig-CasCast}, to generate local details, observation $x_{0:T}$ and the blurry prediction $y^{\prime}_{T:T^{\prime}}$ are first encoded into latent representations $\mathrm{E}(x_{0:T})$ and $\mathrm{E}(y^{\prime}_{T:T^{\prime}})$ as the condition. The conditional distribution of latent diffusion vectors $z_{0:K}$ is factorized and parameterized as:
\begin{equation}
\begin{align}
    % z_{cond}^{x} &= \varepsilon(x_{0:T}) \\
    % z_{cond}^{y^{\star}} &= \varepsilon(y^{\star}_{T:T^{\prime}}) \\
    % p_{\theta}(z_{0:K}|z_{cond}^{x}, z_{cond}^{y^{\star}}) &= p(z_{K}) \prod_{K}^{k=1} p_{\theta}(z_{k-1}|z_{k}, z_{cond}^{x}, z_{cond}^{y^{\star}})
    z_{cond} &= [\mathrm{E}(y^{\prime}_{T:T^{\prime}}),  \mathrm{E}(x_{0:T})] \\
    p_{\theta_{p}}(z_{0:K}|z_{cond}) &= p(z_{K}) \prod_{K}^{k=1} p_{\theta_{p}}(z_{k-1}|z_{k}, z_{cond})
\end{align}
\end{equation}
where $Z_{K} \sim p(z_{k})=N(0,1)$. As proposed by ~\cite{ho2020denoising}, an equivalent parameterization for diffusion models to match the transition state $z_{k-1}$ is predicting the noise $\epsilon_{\theta}(z_k, k)$ of the $k^{th}$ step. The training objective of the diffusion part in CasCast is then simplified to noise prediction loss:
\begin{equation}
\begin{align}
    % z_k &= \sqrt{\Bar{\alpha_k}} z^{y} + \sqrt{1-\Bar{\alpha_k}} \epsilon \\
    % L_{\theta_{p}}(z^{y}, z^{cond})&=E_{\epsilon, k}[||\epsilon - \epsilon_{\theta}(z_{k}, k, z_{cond}) ||_{2}^{2}] \\
    z_k &= \sqrt{\Bar{\alpha_k}}z^y  + \sqrt{1-\Bar{\alpha_k}} \epsilon \\
    L_{\theta_{p}}(z^{y}, z^{cond})&=E_{\epsilon, k}[||\epsilon - \epsilon_{\theta}(z_{k}, k, z_{cond}) ||_{2}^{2}] \\
\end{align}
\end{equation}
where $\epsilon \sim N(0,1)$, $k \sim U(0,1)$ and $z^y=\mathrm{E}(y_{T:T^{\prime}})$.


\subsection{CasFormer}
 We introduce CasFormer for the cascaded generation of precipitation nowcasting. As the generation of the evolution of small-scale precipitation systems is conditioned by the blurry deterministic prediction $y^{\prime}_{T:T^{\prime}}$, there is a frame-by-frame correspondence between  $y^{\prime}_{T:T^{\prime}}$ and the final prediction $y^{\prime\prime}_{T:T^{\prime}}$. Motivated by the correspondence, Our CasFormer generates local details with frame-wise guidance. Specifically, in the process of denoising latent vector $z_k$ to $z_{k-1}$, CasFormer performs frame splitting on the latent representation $\mathrm{E}(y^{\prime}_{T:T^{\prime}})$ of blur prediction and latent vector $z_{k}$. During frame splitting, $z_k$ and $\mathrm{E}(y^{\prime}_{T:T^{\prime}})$ are first split along dimension T into independent frame-wise $\mathrm{E}(y^{\prime}_{T:T^{\prime}})^{j} \in R^{C_z, H_z, W_z}$ and $z_k^j \in R^{C_z, H_z, W_z}$ where $j$ indicates the $j^{th}$ frame in the prediction sequence. Then $\mathrm{E}(y^{\prime}_{T:T^{\prime}})^{j}$ and $z_k^j$  are concatenated along dimension C, resulting frame-wise input $\in R ^{2C_z, H_z, W_z}$. The frame-wise input is utilized to extract the frame-wise feature $h_f^j \in R^{d, h, w}$ with a patch embedding layer and $\frac{L}{2}$ layers of diffusion attention block ~\cite{peebles2023scalable}. Frame-wise features $h_f^0 \dots h_f^{T\prime-T}$ of the same prediction sequence are aggregated into the sequence-wise feature $h_s \in R^{(T^{\prime}-T)\times d^{\prime}, h, w}$ by a sequence aggregator. In the sequence aggregator, frame-wise features are combined as $h_s = MLP(concat(h_f^0 \dots h_f^{T\prime-T}))$, and $h_s$ are injected with information from observations $\mathrm{E}(x_{0:T})$ in the latent space by a cross attention block. In the decoding stage, $h_s$ are decoded into the latent vector $z_{k-1}$ of the $(k-1)^{th}$ step. Overall, CasFormer has a frame-wise encoding stage and a sequence-wise decoding stage. The frame-wise encoding provides better-matched conditions for each frame-wise latent vector, reducing the complexity of the denoising conditioned by a sequence of blurry predictions.  Sequence-wise decoding utilizes the sequence features from the sequence-aggregator to ensure the spatiotemporal consistency of precipitation nowcasting.
